Performance Limits of Neighbor Discovery in Wireless Networks

Neighbor Discovery (ND) is the process employed by two wireless devices to discover each other. There are many different ND protocols, both in the scientific literature and also those employed in practice. All ND protocols involve devices sending beacons, and also listening for them. Protocols differ in terms of how the beacon transmissions and reception windows are scheduled, and the device sleeps in between consecutive transmissions and reception windows in order to save energy. A successful discovery constitutes a sending device's beacon overlapping with a receiving device's reception window. The goal of all ND protocols is to minimize the discovery latency. In spite of the ubiquity of ND protocols and active research on this topic for over two decades, the basic question "Given an energy budget, what is the minimum guaranteed ND latency?", however, still remains unanswered. Given the different kinds of protocols that exist, there has also been no standard way of comparing them and their performance. This paper, for the first time, answers the question on the best-achievable ND latency for a given energy budget. We derive discovery latencies for different scenarios, e.g., when both devices have the same energy budgets, and both devices have different energy budgets. We also show that some existing protocols can be parametrized such that they perform optimally. The fact that the parametrizations of some other protocols were optimal was not known before, and can now be established using our technique. Our results are restricted to the case when a few devices discover each other at a time, as is the case in most real-life scenarios. When many devices need to discover each other simultaneously, packet collisions play a dominant role in the discovery latency and how to analyze such scenarios need further study.

==> sections/app_failure_rate.tex <==
\section{Non-Repetitive Reception Window Sequences}
\label{app:non_repetitive_beacon_sequences}
Throughout this paper, we have restricted our considerations to infinite length reception window sequences $C_\infty$ that are given by concatenations of some finite sequence $C$. Though all currently known deterministic \ac{ND} protocols are constructed accordingly, reception window sequences that continuously alter over time are also feasible.
In what follows, we study such sequences and establish that all our presented bounds remain valid for them.

Let us consider an arbitrary pattern of reception windows of infinite length $C_\infty$. Such a $C_\infty$ is characterized by its reception duty-cycle $\gamma$. As in Section~\ref{sec:analysis}, we consider a sequence $B^\prime$ that consists of those beacons that are sent after both devices have come into range. Obviously, the first beacon $b_1 \in B^\prime$ is received successfully if it directly overlaps with one of the reception windows. The fraction of time-units at which a transmission of $b_1$ leads to a reception is therefore identical to $\gamma$. Another beacon that is sent by $\lambda_1$ time units later leads to additional points in time at which $b_1$ can be sent, such that one beacon out of $b_1, b_2$ is received successfully. These additional points in time lie $\lambda_1$ time-units earlier. Hence, like in Section~\ref{sec:analysis}, such points in time for later beacons are given by translating those of earlier ones temporally to the left.
If every point in time is covered by exactly one such translation, the tuple ($B^\prime, C_\infty$) is disjoint and deterministic, and hence potentially optimal. This holds also true for cases in which $C_\infty$ is not an infinite concatenation of the same $C$. The number of beacons $M$ that need to be sent for guaranteeing deterministic discovery is therefore identical to the number of translations of the reception pattern $C_\infty$, such that every point in time overlaps with exactly one such translation. It is:
\begin{equation}
\label{eq:BeaconingTheoremNonRep}
M = \left\lceil \frac{1}{\gamma} \right\rceil
\end{equation}
\nomenclature{$M$}{Integer value}

The ceiling function in Equation~\ref{eq:BeaconingTheoremNonRep} implies that only reception duty-cycles $\gamma$ that are given by $\nicefrac{1}{k}$, $k = 1,2,3,4,...$ are optimal, since $\gamma$ could be decreased without incurring a larger value of $M$ otherwise.
Hence, optimal protocols are composed of deterministic beacon sequences $B^\prime$ of length $M = \nicefrac{1}{\gamma}$, since $\nicefrac{1}{\gamma}$ will always be an integer-value. The same considerations as in Theorem~\ref{thm:worst_case_latency_theorem} lead to the following bound:
\begin{equation}
\label{eq:BoundUniDirNonRep}
L = \frac{\omega}{\beta \gamma}
\end{equation}
This is equivalent to Theorem~\ref{eq:boundUnidir}, from which all further bounds are derived. Hence, all our bounds remain valid for non-repetitive reception window sequences. 



\section{Failures due to Collisions}
\label{app:failure_rate}
A limit on the channel utilization often results from minimizing the rate of failed discoveries for a larger number of devices. For such large networks, what is the best relation between the duty-cycle, the discovery latency and the probability using which this discovery latency is achieved? And which limit on the channel-utilization results from this relation? A \ac{ND} protocol that performs optimal in this trade-off can at the same time potentially guarantee a low worst-case latency for a pair of two devices (for which collisions do not occur), which is determined by the channel utilization.
While we have studied the impact of the channel utilization on the theoretic worst-case lateny bound for a pair of devices in Section~\ref{sec:collision_constrained_discovery}, we below study which latency can be achieved with a given failure-rate for a given duty-cycle in large networks.

In networks in which multiple devices carry out the \ac{ND} procedure simultaneously, collisions are inevitable and the theoretical worst-case latency $L$ is only achieved with a certain probability. In such cases, a \ac{ND} protocol is characterized by a latency function $L^\prime(\eta, P_f, S)$. The latency $L^\prime$ is the lowest latency that is not exceeded by more than a fraction of $P_f$ of all discovery attempts. This means that when $S$ devices attempt to discover each other, a fraction of $1 - P_f$ of all discovery attempts will be successful within $L^\prime$ time-units. The remaining attempts will either be successful at a later point in time or fail permanently. The question we study in this section is: Given a certain tuple $(\eta, P_f, S)$, what is the best $L^\prime$ that can be achieved?

When not accounting for collisions (i.e., in the two-node case considered in Section~\ref{sec:bounds}), the optimum for $L$ is achieved by covering every possible initial offset exactly once, i.e., $\Lambda = T_C$. Let us now consider \ac{ND} protocols in which  certain offsets are covered multiple times. This can be realized using beacon sequences that are extensions of shorter, non-redundant sequences, i.e., every offset is first covered once by a short sequence that minimizes $L$ and then covered again by later beacons that apply if an earlier one has collided. Towards this, let us consider a parameter  $q \in [0, 1]$ and a second parameter $Q \in \mathbb{Z}$. A fraction $q$ of all offsets is covered $Q+1$ times and the remaining offsets are covered $Q$ times. We further assume that a collision of any two beacons occurs entirely independent of any previous collision, e.g., the collision probability is $P_C$ for \textit{every} pair of beacons. It is not clear whether beacon sequences that actually fulfill this assumption can be designed, but such a complete decorrelation represents the theoretic optimum. With $P_c = 1 - e^{-2(S-2)\beta}$, the failure rate is given by the following equation:
\begin{equation}
P_f = (1-q)(1 - e^{-2(S-2)\beta})^Q + q (1 - e^{-2(S-2)\beta})^{Q+1}
\end{equation}
\nomenclature{$P_f$}{Rate using which discovery fails due to collisions}
\nomenclature{$L^\prime$}{Latency bound that can be achieved given a certain failure rate $P_f$ among $S$ devices.}
\nomenclature{$Q$}{Factor using which every offset is covered redundantly}
\nomenclature{$q$}{Fraction of offsets that are covered reduntantly by one instance more than $Q$}

Here, $S-2$ senders are relevant for the collision probability, because the beacons from every pair of devices discovering each other can never collide with themselves, but with the beacons from further devices. Solving this equation by $\beta$ is only easily possible for $q = 0$ - for other values, numeric solutions are feasible. Assuming $q=0$ implies that the amount of redundancy that is optimal can only be approximated using the integer-value $Q$. The resulting near-optimal value of $\beta$ can be inserted into the following modified form of Equation~\ref{eq:wc_latency_theorem}, which accounts for every initial offset being covered $Q$ times. 
\begin{equation}
L(P_f) = \left \lceil \frac{Q \cdot T_C}{\sum_{i=1}^{n_C} d_{i}} \right \rceil \frac{\omega}{\beta}
\end{equation} 
For example, when assuming $\omega = \SI{36}{\micro s}, \alpha = 1, \eta = \SI{5}{\percent}, P_f = \SI{0.05}{\percent}, S = 3$, the optimal value of $Q$ is $3$ and $L(P_f) = \SI{0.1583}{s}$. The resulting channel utilization is $\SI{2.07}{\percent}$, which leads to a theoretical worst-case latency $L$ for a pair of nodes of $\SI{0.05}{s}$. For 3 nodes, $L$ is not reached by $P_c = \SI{7.9}{\percent}$ of all discovery attempts.
However, $L^\prime$ can only be achieved under the assumption that all beacons of multiple devices collide independently from each other. It is currently not known whether such perfectly uncorrelated sequences can be designed.

==> sections/app_low_power_listening_transmit.tex <==
\section{Low Power Listening/Transmit}
\label{app:low_power_listening_transmit}
Some protocols, e.g., U-Connect \cite{Kandhalu:10}, make use of a technique known as \textit{low power listening/transmit}. Instead of sending short beacons that need to overlap with relatively longer reception phases, they use contiguous transmission phases that are significantly larger than one beacon transmission duration. The reception phases for detecting these beacons can in turn become as short as the hardware supports. Such protocols can be described by interchanging beacons and reception windows in the model presented above. Thereby, reception window sequences are used to model transmissions, whereas beacon sequences describe the radio's reception pattern.


==> sections/app_unideal_radios.tex <==
\section{Radio Overheads}
\label{sec:radio_overheads}
Throughout this paper, we have assumed that the radios do not require any energy to switch from sleep mode to transmission or reception, and vice-versa. In this section, we outline how the fundamental bounds change when such energy overheads are considered. Let us assume an overhead $d_{oTx}$ to switch the radio from the sleep mode to transmission and back, and an overhead $d_{oRx}$ to switch from the sleep mode to reception and back. These overheads can be regarded as effective additional durations of active time, i.e., as the actual durations that are needed to switch the radio's mode of operation, weighted by the quotient of the average power consumption during the switching phase over the power consumption for reception.

When accounting for these offsets, one can derive from Equation~\ref{eq:etaRegular} that the duty-cycle for transmission of repetitive sequences becomes: 
\begin{equation}
\beta = \sum_{i=1}^{m_B} \frac{\omega_i + d_{oTx}}{\lambda_i}
\end{equation}
Similarly, the duty-cycle for reception becomes:
\begin{equation}
\gamma = \frac{\sum_{i=1}^{m_B}(d_i + d_{oRx})}{T_C}
\end{equation}
With this, Theorem~\ref{eq:boundUnidir} for unidirectional beaconing, from which all other bounds are derived, becomes:
\begin{equation}
L = \frac{1}{\gamma} \cdot \left(1 + \frac{\sum_{i=1}^{n_C} d_{oRx}}{\sum_{i=1}^{n_C} d_{i}}\right) \cdot \frac{\omega + d_{oTx}}{\beta}.
\end{equation}
Note that the worst-case latency depends on the number of reception windows $n_C$, which needs to be minimized to get the tightest latency bound. Therefore, sequences that consist of one single, large reception window per period $T_C$ are most efficient.
With this reception window having a length of $d_1$, the bound for unidirectional beaconing, from which all further bounds can be derived in the way described in the paper, is as follows:
\begin{equation}
L = \frac{1}{\gamma} \cdot \left(1 + \frac{d_{oRx}}{d_{1}}\right) \cdot \frac{\omega + d_{oTx}}{\beta}.
\end{equation}
\nomenclature{$d_{oTx}$}{Effective additional active time for switching from sleep to transmission and vice-versa}
\nomenclature{$d_{oRx}$}{Effective additional active time for switching from sleep to reception and vice-versa}
In addition, a non-ideal radios incurs a similar overhead $d_{oTxRx}$ to switch from transmission to reception and an overhead $d_{oRxTx}$ to switch from reception to transmission. The implications of these overheads are described in Appendix~\ref{{app:nonOverlappingSequences}.


==> sections/app_unidir.tex <==
\section{Mutual Exclusive Unidirectional Discovery}
\label{sec:correlatedSchedules}
\begin{figure}[bt]
	\centering
	\includegraphics[width=\linewidth]{images/crossCorrellations.png}
	\caption{Correlated offsets $\Phi_{F,1}$ and $\Phi_{E,1}$ in the sequences of two devices \textit{E} and \textit{F}.}
	\label{fig:crossCorrelation} 
\end{figure}
In Section~\ref{sec:uniDirBeaconing}, we have studied unidirectional discovery in the sense that one device~\textit{F} could discover \textit{E} without \textit{E} discovering \textit{F}. However, it is also possible to design the tuple $(B_\infty, C_\infty)$ on each device such that either device~\textit{E} or \textit{F} can directly discover its opposite, which we study in this section.

This form of unidirectional discovery is realized using beacon sequences $B \in B_\infty$, in which the beacons on one device are sent with a fixed temporal relation to the reception windows on the same device. For example, let beacon $b_{F,1}$ on device~\textit{F} be sent by $\zeta$ time-units after reception window $X_{F,1}$, as depicted in Figure~\ref{fig:crossCorrelation}. Further, let such a relation exist on both devices and in every period $T_C$ of the reception window sequence. As previously explained $b_{F,1}$ has a random offset of $\Phi_{F,1}$ time-units from the coordinate origin of device~\textit{E}. The temporal correlation between $B_\infty$ and $C_\infty$ on every device implies that the offset $\Phi_{E,1}$ beacon $b_{E,1}$ has from the coordinate origin of device~\textit{F} is fully determined by $\Phi_{F,1}$ (cf. Figure~\ref{fig:crossCorrelation}). It is:
\begin{equation}
\label{eq:crossCorrelation}
\Phi_{E,1} = \zeta + (\zeta - \Phi_{F,1}) = 2 \cdot \zeta - \Phi_{F,1}
\end{equation}
\nomenclature{$\zeta$}{Fixed temporal distance of a certain beacon from a certain reception window on the same device in every period $T_C$}

By exploiting this temporal relation, a quadruple of sequences $(C_{F,\infty},B_{E,\infty}, C_{E,\infty}, B_{F,\infty})$ can guarantee deterministic one-way discovery, even if the pair $(C_{E,\infty}, B_{F,\infty})$ only covers half of the offsets $\Phi_{F,1} \in [0, T_C]$, by having the pair $(C_{F,\infty}, B_{E,\infty})$ covering the remaining ones. Thereby, the number of beacons that need to be sent per device for guaranteeing one-way discovery can be halved.
\begin{figure}[tb]
	\centering
	\includegraphics[width=\linewidth]{images/mutualAssistance.png}
	\caption{Quadruple of sequences $\mathbf{(C_{E,\infty}, B_{E,\infty},}$ $\mathbf{C_{F,\infty}, B_{F,\infty})}$ that exploits temporal correlations.% Hatched beacons and grayed-out coverage images correspond to beacons that are not send, but their transmission would be necessary in uncorrelated schedules.
	}
	\label{fig:crossCorrelatedSchedule} 
\end{figure}
The upper part of Figure~\ref{fig:crossCorrelatedSchedule} depicts the beacons (arrows) and reception windows (rectangles) of two devices \textit{E} and \textit{F}. On each device, the reception windows and beacons have a fixed temporal relation, whereas beacon $b_{F,1}$ has a random offset $\Phi_{F,1}$ from the coordinate origin of device~\textit{E}. Dashed arrows depict beacons that would need to be sent if every device would have to cover all offsets in the entire period $T_C$ on its own. When exploiting temporal correlations between $B_\infty$ and $C_\infty$ on the same device, these beacons can be omitted without increasing the one-way worst-case latency. The lower part of Figure~\ref{fig:crossCorrelatedSchedule} depicts the coverage map of the beacons $b_{F,1},...,b_{F,4}$ of device~\textit{F} and $b_{E,1},...,b_{E,4}$ of device~\textit{E}. 
This coverage map represents all offsets $\Phi_{F,1}$, for which either a beacon from device~\textit{F} overlaps with a reception window of device~\textit{E} or a beacon from device~\textit{E} overlaps with a reception window of device~\textit{F}.
Covered offsets of omitted beacons have been left white. As can be seen, every possible initial offset $\Phi_{F,1}$ is covered by either a beacon of $B_{F,\infty}$ falling into a reception window of $C_{E,\infty}$, or a beacon of $B_{E,\infty}$ falling into a reception window of $C_{F,\infty}$, and hence the number of beacons per device is halved compared to direct bi-directional discovery. This leads to the following latency bound, which is lower than the one given by Theorem~\ref{thm:boundSymUncorrelated}. Since there are no further possibilities to improve pairwise discovery, this is also the tightest fundamental bound for all pairwise deterministic \ac{ND} protocols.

\begin{theorem}
\label{thm:boundCorrelated}

The lowest worst-case latency a pair of devices can guarantee for mutual exclusive one-way discovery  (i.e., either of both devices can discover its opposite one) is given by:
\begin{equation}
\label{eq:boundCorrelated}
L = \min\left(\left\lceil \frac{1}{\eta} \right\rceil^2 \cdot \frac{\omega \alpha}{\eta \cdot \lceil \nicefrac{1}{\eta} \rceil  - 1/2}, \left\lfloor \frac{1}{\eta} \right\rfloor^2 \cdot \frac{\omega \alpha}{\eta \cdot \lfloor \nicefrac{1}{\eta} \rfloor - 1/2}\right)
\end{equation}
\begin{prf}
For a given set of offsets $\Omega_{F}$ covered by $B_{F} \in B_{F,\infty}$ on device~\textit{E}, Equation \ref{eq:crossCorrelation} defines a set of offsets $\Omega_{E}$ that are automatically covered by $B_{E} \in B_{E,\infty}$ on device $F$, and vice-versa. 
If $\Omega_F$ and $\Omega_E$ are disjoint, the amount of offsets contained in $\Omega_F \cup \Omega_E$ must sum up to $T_C$ time-units for guaranteeing one-way discovery. Hence, the beacon sequence on every device needs to cover only $\nicefrac{1}{2} \cdot T_C$ time-units to guarantee one-way determinism, and Equation~\ref{eq:wc_latency_theorem} becomes:

\begin{equation}
L = \left \lceil \frac{T_C}{2 \cdot \sum_{k=1}^{n_C} d_{k}} \right \rceil \frac{\omega}{\beta}
\end{equation}
The rest of this proof is identical to the one for direct symmetric discovery (cf. Theorem \ref{thm:boundSymUncorrelated}).
\end{prf}
\end{theorem}
Theorem~\ref{thm:boundCorrelated} is valid for one-way discovery (i.e., device~\textit{E} discovers device~\textit{F} \textbf{or} vice-versa). An indirect reverse discovery can be realized as follows. Each device transmits its next point in time at which it listens to the channel along with its beacons. The receiving device then schedules an additional beacon at the received point in time. This technique is called \textit{mutual assistance}~\cite{kindt:17a}, and is actually a form of synchronous connectivity. Here, the latency for two-way discovery will be increased by the maximum temporal distance between any beacon and its succeeding reception window on the same device. An upper bound for this penalty for two-way discovery is $T_C$ time units, which can be reduced significantly in sequences with more than one reception window per period $T_C$.


==> sections/glossary.tex <==
\newacronym{MANET}{MANET}{mobile ad-hoc network}
\newacronym{ND}{ND}{neighbor discovery}
\newacronym{BLE}{BLE}{Bluetooth Low Energy}
\newacronym{PI}{PI}{periodic interval}
